Verifying Transactional Consistency of MongoDB

MongoDB is a popular general-purpose, document-oriented, distributed NoSQL database. It supports transactions in three different deployments: single-document transactions utilizing the WiredTiger storage engine in a standalone node, multi-document transactions in a replica set which consists of a primary node and several secondary nodes, and distributed transactions in a sharded cluster which is a group of multiple replica sets, among which data is sharded. A natural and fundamental question about MongoDB transactions is: What transactional consistency guarantee do MongoDB Transactions in each deployment provide? However, it lacks both concise pseudocode of MongoDB transactions in each deployment and formal specification of the consistency guarantees which MongoDB claimed to provide. In this work, we formally specify and verify the transactional consistency protocols of MongoDB. Specifically, we provide a concise pseudocode for the transactional consistency protocols in each MongoDB deployment, namely WIREDTIGER, REPLICASET, and SHARDEDCLUSTER, based on the official documents and source code. We then prove that WIREDTIGER, REPLICASET, and SHARDEDCLUSTER satisfy different variants of snapshot isolation, namely Strong-SI, Realtime-SI, and Session-SI, respectively. We also propose and evaluate efficient white-box checking algorithms for MongoDB transaction protocols against their consistency guarantees, effectively circumventing the NP-hard obstacle in theory.

==> algs/check/check.tex <==
% check.tex

\begin{algorithm}[t]
    \caption{MongoDB Snapshot Isolation Checking Algorithm}
    \label{alg:si-check}
    \begin{algorithmic}[1]
        %% Is some si variant
        % \Procedure{\issomesivariant}{$\hisvar, \sivariantvar, \visvar, \arvar$}
        % \label{alg:issomesivariant}
        % \If{$\visvar$ is not strict partial order}
        % \State \Return \false
        % \EndIf
        % \If{$\arvar$ is not strict total order}
        % \State \Return \false
        % \EndIf
        % \State $\axiomsvar \gets $ corresponding axioms of $\sivariantvar$
        % \For{$\axiomvar \in \axiomsvar$}
        % \If{$(\hisvar,\visvar,\arvar) \nvDash \axiomvar$.}
        % \State \Return \false
        % \EndIf
        % \EndFor
        % \State \Return \true
        % \EndProcedure

        %% Is Strong-SI for wiredtiger
        \Statex
        \Procedure{\isstrongsi}{$\hisvar, \committimewt, \starttimewt, \tidlogsvar$}
        \label{alg:isstrongsi}
        \State $\visvar \gets \emptyset, \arvar \gets \emptyset, \errorvar \gets 0$

        \For{$\txnvar_1 \in \hisvar$}
        \For{$\txnvar_2 \in \hisvar$}
        \If{$\committimewt(\txnvar_1) < \starttimewt(\txnvar_2)$}
        \State $\visvar \gets \visvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \ElsIf{$\txnvar_2$ reads from $\txnvar_1$}
        \State $\visvar \gets \visvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \label{line:read-fron-ar}
        \State $\errorvar \gets \max{(\errorvar, \committimewt(\txnvar_2) - \starttimewt(\txnvar_1))}$
        \EndIf

        \If{$\txnvar_1$ conflicts with $\txnvar_2 \land \tidlogsvar(\txnvar_1) < \tidlogsvar(\txnvar_2)$}
        \State $\arvar \gets \arvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \label{line:tid-fix-ar}
        \ElsIf{$\committimewt(\txnvar_1) < \committimewt(\txnvar_2)$}
        \State $\arvar \gets \arvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \EndIf


        \EndFor
        \EndFor

        \State \Return \issomesivariant($\hisvar, \strongsi, \visvar^+, \arvar^+$)

        \EndProcedure

        %% Is SI for MongoDB
        \Statex
        \Procedure{\ismongodbsi}{$\hisvar, \committime, \readtime, \sivariantvar$}
        \label{alg:ismongodbsi}
        \State $\visvar \gets \emptyset, \arvar \gets \emptyset$

        \For{$\txnvar_1 \in \hisvar$}
        \For{$\txnvar_2 \in \hisvar$}
        \If{$\txnvar_1$ is not read only $\land \committime(\txnvar_1) < \readtime(\txnvar_2)$}
        \State $\visvar \gets \visvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \ElsIf{$\txnvar_1$ executes before in the same session with $\txnvar_2$}
        \State $\visvar \gets \visvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \EndIf

        \EndFor
        \EndFor

        \State $\updatesvar \gets $ the update transactions in $hisvar$
        \State $\readonlyvar \gets $ the read only transactions in $hisvar$

        \For{$\txnvar_1 \in \updatesvar$}
        \For{$\txnvar_2 \in \updatesvar$}
        \If{$\committime(\txnvar_1) < \committime(\txnvar_2)$}
        \State $\arvar \gets \arvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \ElsIf{$\committime(\txnvar_1) = \committime(\txnvar_2) \land \txnvar_1.\sidvar < \txnvar_2.\sidvar$}
        \label{line:thesamecommitts}
        \State $\arvar \gets \arvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \EndIf
        \EndFor
        \EndFor


        \For{$\txnvar_1 \in \hisvar$}
        \For{$\txnvar_2 \in \readonlyvar$}
        \If{$(\txnvar_1,\txnvar_2) \in \visvar$}
        \State $\arvar \gets \arvar \cup \set{(\txnvar_1, \txnvar_2)}$
        \EndIf
        \EndFor
        \EndFor

        \State \Return \issomesivariant($\hisvar, \sivariantvar, \visvar^+, \arvar^+$)
        \EndProcedure

        %% Is Realtime-SI for Replica Set
        \Statex
        \Procedure{\isrealtimesi}{$\hisvar, \committimers, \readtimers$}
        \label{alg:isrealtimesi}
        \State \Return \ismongodbsi($\hisvar, \committimers, \readtimers, \rtsi$)
        \EndProcedure

        %% Is Session-SI for Sharded Cluster
        \Statex
        \Procedure{\issessionsi}{$\hisvar, \committimesc, \committimesc$}
        \label{alg:issessionsi}
        \State \Return \ismongodbsi($\hisvar, \committimesc, \committimesc, \sessionsi$)
        \EndProcedure
    \end{algorithmic}
\end{algorithm}


==> algs/rs/clock.tex <==
% clock.tex

\begin{algorithm}[t]
  \caption{Cluster time management.}
  \label{alg:clock}
  \begin{algorithmic}[1]
    % \Statex Hybrid logical clocks are compared lexicographically:
    % \begin{align*}
    %   hlc_{1} = hlc_{2} \iff &(hlc_{1}.sec = hlc_{2}.sec)\; \land \\
    %           &(hlc_{1}.counter = hlc_{2}.counter).
    % \end{align*}
    % \vspace{-0.80cm}
    % \begin{align*}
    %   &hlc_{1} < hlc_{2}\iff  (hlc_{1}.sec < hlc_{2}.sec)\; \lor \\
    %       &\hspace{5pt}(hlc_{1}.sec = hlc_{2}.sec \;\land hlc_{1}.counter < hlc_{2}.counter).
    % \end{align*}

    \Procedure{\tick}{\null}
      \label{line:procedure-tick}
      \If{$\ct.\sec \geq \clock$} \Comment{\red{description of \clock???}}
        \label{line:tick-sec-clock}
        \State \Return $\langle \ct.\sec, \ct.\counter + 1 \rangle$
        \label{line:tick-counter}
      \Else
        \State \Return $\langle \clock, 0 \rangle$
        \label{line:tick-clock}
      \EndIf
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> algs/rs/rs-app.tex <==
% rsapp.tex

\begin{algorithm}[p]
  \caption{\rsapp: the application code}
  \label{alg:rs-app}
  \begin{algorithmic}[1]
    \State
  \end{algorithmic}
\end{algorithm}


==> algs/rs/rs-client.tex <==
% rs-client.tex

\begin{algorithm}[t]
  \caption{\rsalg: the client library}
  \label{alg:rs-client}
  \begin{algorithmic}[1]
    \Procedure{\rsclopen}{\null}
      \label{line:procedure-rsclopen}
      \State establish a connection to the primary
        \label{line:rsclopen-connection}
      \State $\rssidvar \gets \Call{\uuid}{\null}$
        \label{line:rsclopen-rssid}
      \State $\rssessionvar \gets \tuple{\rssidvar, \false}$
        \label{line:rsclopen-rssession}
      \State \Return $\rssessionvar$
        \label{line:rsclopen-return}
    \EndProcedure

    % \Statex
    \Procedure{\rsclstart}{$\rssessionvar$}
      \label{line:procedure-rsclstart}
      \State $\rssessionvar.\isstartingtxn \gets \true$
        \label{line:rsclstart-isstartingtxn}
      \State \Return $\rssessionvar$
        \label{line:rsclstart-return}
    \EndProcedure

    % \Statex
    \Procedure{\rsclread}{$\rssessionvar, \keyvar$}
      \label{line:procedure-rsclread}
      \State $\tuple{\rssessionvar, \valvar} \gets \rpc \rsread(\rssessionvar, \keyvar)$
        \label{line:rsclread-call-rsread}
      \State \Return $\tuple{\rssessionvar, \valvar}$
        \label{line:rsclread-return}
    \EndProcedure

    % \Statex
    \Procedure{\rsclupdate}{$\rssessionvar, \keyvar, \valvar$}
      \label{line:procedure-rsclupdate}
      \State $\tuple{\rssessionvar, \statusvar} \gets \rpc \Call{\rsupdate}{\rssessionvar, \keyvar, \valvar}$
        \label{line:rsclupdate-call-rsupdate}
      \State \Return $\tuple{\rssessionvar, \statusvar}$
        \label{line:rsclupdate-return}
    \EndProcedure

    % \Statex
    \Procedure{\rsclcommit}{$\rssessionvar$}
      \label{line:procedure-rsclcommit}
      \State $\_ \gets \rpc \Call{\rscommit}{\rssessionvar}$
        \label{line:rsclcommit-call-rscommit}
      \State \Return \ok
        \label{line:rsclcommit-return}
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> algs/sc/sc-client.tex <==
% sc-client.tex

\begin{algorithm}[tbp]
  \caption{\scalg: the client library}
  \label{alg:sc-client}
  \begin{algorithmic}[1]
    \Procedure{\scclopen}{\null}
      \label{line:procedure-scclopen}
      \State $\scsidvar \gets \rpc \Call{\scmongosopen}{\null}$
        \label{line:scclopen-call-scmongosopen}
      \State \Return $\scsidvar$
        \label{line:scclopen-return}
    \EndProcedure

    % \Statex
    % \Procedure{\scclstart}{$\scsidvar$}
    %   \label{line:procedure-scclstart}
    %   \State $\rpc \scmongosstart(\scsidvar)$
    %     \label{line:scclstart-call-scmongosstart}
    %   \State \Return \ok
    %     \label{line:scclstart-return}
    % \EndProcedure

    % \Statex
    \Procedure{\scclread}{$\scsidvar, \keyvar$}
      \label{line:procedure-scclread}
      \State $\valvar \gets \rpc \scmongosread(\scsidvar, \keyvar)$
        \label{line:scclread-call-scmongosread}
      \State \Return $\valvar$
        \label{line:scclread-return}
    \EndProcedure

    % \Statex
    \Procedure{\scclupdate}{$\scsidvar, \keyvar, \valvar$}
      \label{line:procedure-scclupdate}
      \State $\statusvar \gets \rpc \Call{\scmongosupdate}{\scsidvar, \keyvar, \valvar}$
        \label{line:scclupdate-call-scmongosupdate}
      \State \Return $\statusvar$
        \label{line:scclupdate-return}
    \EndProcedure

    % \Statex
    \Procedure{\scclcommit}{$\scsidvar$}
      \label{line:procedure-scclcommit}
      \State $\decvar \gets \rpc \Call{\scmongoscommit}{\scsidvar}$
        \label{line:scclcommit-call-scmongoscommit}
      \State \Return $\decvar$
        \label{line:scclcommit-return}
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> algs/sc/sc-mongos.tex <==
% sc-mongos.tex

\begin{algorithm}[p]
  \caption{\scalg: the mongos}
  \label{alg:sc-mongos}
  \begin{algorithmic}[1]
    \Procedure{\scmongosopen}{\null}
      \label{line:procedure-scmongosopen}
	  \State \Return \Call{\uuid}{\null}
	    \label{line:scmongosopen-return}
    \EndProcedure

    \Statex
    \Procedure{\scmongosread}{$\scsidvar, \keyvar$}
      \label{line:procedure-scmongosread}
      \State $\shardidvar \gets \shardof(\keyvar)$
        \label{line:scmongosread-shardid}
      \State $\fieldsvar \gets \continue(\scsidvar, \shardidvar)$
        \label{line:scmongosread-call-continue}
      \State $\tuple{\valvar, \scrsconnsvar} \gets \send
        \scread(\scsidvar, \keyvar, \fieldsvar) \sendto \primaryof(\shardidvar)$
        \label{line:scmongosread-call-scread}
      \State $\scrsconns \gets \scrsconnsvar$
        \label{line:scmongosread-scrsconns}
      \State \Return $\valvar$
        \label{line:scmongosread-return}
    \EndProcedure

    \Statex
    \Procedure{\scmongosupdate}{$\scsidvar, \keyvar, \valvar$}
      \label{line:procedure-scmongosupdate}
      \State $\routervar \gets \scroutertable[\scsidvar]$
        \label{line:scmongosupdate-router}
      \State $\shardidvar \gets \shardof(\keyvar)$
        \label{line:scmongosupdate-shardid}
      \State $\fieldsvar \gets \continue(\scsidvar, \shardidvar)$
        \label{line:scmongosupdate-call-continue}
      \State $\tuple{\statusvar, \scrsconnsvar} \gets \send \scupdate(\scsidvar, \keyvar, \fieldsvar) \sendto \primaryof(\shardidvar)$
        \label{line:scmongosupdate-call-scupdate}
      \State $\scrsconns \gets \scrsconnsvar$
        \label{line:scmongosupdate-scrsconns}
      \If{$\statusvar = \ok$}
        \label{line:scmongosupdate-status-if-ok}
        \State $\routervar.\readonly \gets \false$
          \label{line:scmongosupdate-router-readonly}
      \Else
        \label{line:scmongosupdate-status-if-rollback}
        \State $\send \Call{\abort}{\scsidvar} \sendto \primaryvar \in \primaryof(\routervar.\participants \setminus \set{\shardidvar})$
          \label{line:scmongosupdate-call-abort}
      \EndIf
      \State \Return $\statusvar$
        \label{line:scmongosupdate-return}
    \EndProcedure

    \Statex
    \Procedure{\scmongoscommit}{$\scsidvar$}
      \label{line:procedure-scmongoscommit}
      \State $\routervar \gets \scroutertable[\scsidvar]$
        \label{line:scmongoscommit-router}
      \State $\participantsvar \gets \routervar.\participants$
        \label{line:scmongoscommit-participant}
      \If{$\participantsvar = \emptyset$}
        \label{line:scmongoscommit-router-participants-empty}
        \State \Return \ok
          \label{line:scmongoscommit-return-no-participants}
      \EndIf
      \If{$|\participantsvar| = 1 \lor \routervar.\readonly$}
        \label{line:scmongoscommit-router-one-participant}
        \State $\_ \gets \send \Call{\rscommit}{\scrsconns[\scsidvar]} \sendto \participantvar \in \primaryof(\participantsvar)$
          \label{line:scmongoscommit-call-directcommit}
          \State \Return \ok
            \label{line:scmongoscommit-return-single-readonly}
      \EndIf

      % \State $\coordvar \gets \primaryof(\routervar.\coord)$
      %   \label{line:scmongoscommit-coord}
      \State $\twopcack(\decvar) \gets \send \Call{\twopc}{\scsidvar, \participantsvar} \sendto \primaryof(\routervar.\coord)$
        \label{line:scmongoscommit-call-twopc}
      % \State $\wait\receive \Call{\twopcack}{\statusvar} \from \coordvar$
      %   \label{line:scmongoscommit-call-twopcack}
      \State \Return $\decvar$
        \label{line:scmongoscommit-return-twopc}
    \EndProcedure

    \Statex
    \Procedure{\continue}{$\scsidvar, \shardidvar$}
      \label{line:procedure-continue}
      \State $\fieldsvar \gets [\iscoord \mapsto \false,
        \isstartingtxn \mapsto \true, \atclustertime \mapsto \wttsnone]$
        \label{line:continue-field}

      \hStatex
      \State $\routervar \gets \scroutertable[\scsidvar]$
        \label{line:continue-router}
      \If{$\routervar.\participants = \emptyset$}
        \label{line:continue-if-router-participants}
        \State $\routervar.\coord \gets \shardidvar$
          \label{line:continue-router-coordid}
        \State $\routervar.\atclustertime \gets \ct$
          \label{line:continue-router-atclustertime}
        \State $\fieldsvar.\iscoord \gets \true$
          \label{line:continue-field-iscoord}
      \EndIf

      \If{$\shardidvar \in \routervar.\participants$}
        \label{line:continue-if-shardid}
        \State $\fieldsvar.\isstartingtxn \gets \false$
          \label{line:continue-field-isstartingtxn}
      \Else
        \State $\routervar.\participants \gets @ \cup \set{\shardidvar}$
          \label{line:continue-router-participants}
      \EndIf
      \State $\fieldsvar.\atclustertime \gets \routervar.\atclustertime$
        \label{line:continue-field-atclustertime}

      \State \Return $\fieldsvar$
        \label{line:continue-return}
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> algs/wt/wt-client.tex <==
% wt-client.tex

\begin{algorithm}[p]
  \caption{\wtalg: the client side}
  \label{alg:wt-client}
  \begin{algorithmic}[1]
    \Procedure{\wtclopen}{\null}
      \label{line:procedure-opensession}
      \State $\wtsidvar \gets \Call{}{}$
      \State $\wtsession \gets \tuple{\wtsidvar, \tuple{0, 0, 0, \emptyset, \emptyset}}$
      \State \Return \ok
    \EndProcedure

    \Statex
    \Procedure{\wtclstart}{\null}
      \label{line:procedure-starttx}
      \State $\wtsession \gets \Call{\wtstart}{\wtsession}$
      \State \Return \ok
    \EndProcedure

    \Statex
    \Procedure{\wtclread}{$\keyvar$}
      \label{line:procedure-wtreadkey}
      \State \Return $\Call{\wtread}{\wtsession, \keyvar}$
    \EndProcedure

    \Statex
    \Procedure{\wtclupdate}{$\keyvar, \valvar$}
      \label{line:procedure-wtupdatekey}
      \State \Return $\Call{\wtupdate}{\wtsession, \keyvar, \valvar}$
    \EndProcedure

    \Statex
    \Procedure{\wtclcommit}{\null}
      \label{line:procedure-committx}
      \State \Return $\Call{\wtcommit}{\wtsession}$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> figs/fig-axioms.tex <==
% fig-axioms.tex

\begin{figure*}[tbhp]
  \centering
  \begin{align}
    \tag{\intaxiom} \label{axiom:int} \\
    \tag{\extaxiom} \label{axiom:ext} \\
    \sorel \subseteq \vis
      \tag{\sessionaxiom} \label{axiom:session} \\
    \ar \comp \vis \subseteq \vis
      \tag{\prefixaxiom} \label{axiom:prefix} \\
    \forall S, T \in \h.\; S \conflict T \implies (S \rel{\vis} T \lor T \rel{\vis} S)
    \tag{\noconflictaxiom} \label{axiom:noconflict} \\
    \forall S, T \in \h.\; S \rel{\vis} T \implies \starttime(T) > \committime(S)
      \tag{\inrbaxiom} \label{axiom:realtimesnapshot} \\
    \rb \subseteq \vis
      \tag{\rbaxiom} \label{axiom:rb} \\
    \cb \subseteq \ar
      \tag{\cbaxiom} \label{axiom:cb}
  \end{align}
  \caption{Consistency axioms, constraining an abstract execution $(\h, \vis, \ar)$.}
  \label{fig:axioms}
\end{figure*}


==> figs/fig-check-perf-norm.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figs/tikz/check-mongo-perf/check-mongo-perf.pdf}
    \caption{The MongoDB deployment.}
    \label{fig:si-check-perf}
\end{figure*}


==> figs/fig-example-read-commit-ts.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figs/tikz/read-commit-timestamp/read-commit-timestamp}
    \caption{Read timestamps at different times in Example~\ref{ex:read-commit-ts}.
        \red{Explain: color just for more readable, tid is enough to classify.}}
    \label{fig:ex:read-commit-ts}
\end{figure*}


==> figs/fig-example-snapshot.tex <==
\begin{figure*}
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/tikz/consistent-snapshot/clock-skew}
        \subcaption{\caseclockskew{} and \caseholes{}.}
        \label{fig:ex:clock-skew}
    \end{minipage}
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/tikz/consistent-snapshot/pending-commit}
        \subcaption{\casependingcommitread{}.}
        \label{fig:ex:pending}
    \end{minipage}

    \caption{The \red{consistent snapshot} in Example~\ref{ex:sc-snapshot}.}
    \label{fig:ex:sc-snapshot}
\end{figure*}


==> figs/fig-mongo-txn-number.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figs/tikz/mongo-stat/mongo-stat.pdf}
    \caption{The MongoDB deployment.}
    \label{fig:wt-mongo-num}
\end{figure*}


==> figs/fig-wt-txn-number.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figs/tikz/wt-stat/wt-stat.pdf}
    \caption{Statistics of executed transactions.}
    \label{fig:wt-txn-num}
\end{figure*}


==> proofs/rs-correctness.tex <==
% rs-correctness.tex

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness} \label{ss:rs-correctness}

For a relation $R$, we use $R_{\textsc{rs}}$
to denote an instantiation of $R$ specific to the \rsalg{} protocol.
Consider a history $\h = (\RSTXN, \sors)$ of \rsalg{},
where we restrict $\RSTXN$ to be set of \emph{committed} transactions.
Denote by $\RSTXNUPDATE \subseteq \RSTXN$ be the set of update transactions in $\RSTXN$.
We prove that $\h$ satisfies \rtsi{}
by constructing an abstract execution $\ae = (\h, \visrs, \arrs)$
(Theorem~\ref{thm:rsalg-rtsi})
%%%%%%%%%%%%%%%
% \subsubsection{Invariants} \label{sss:rs-invariants}
%
% \begin{enumerate}[(\inv 1)]
%   \item \label{inv:committs-unique}
%     uniqueness of $\committs$
%   \item \label{inv:committs-monotonic}
%     monotonicity of $\committs$
%   \item \label{inv:rs-ts-wttxnglobal}
%     Let $\tuple{\_, \tsvar}$ be a value of
%     $\wttxnglobal[\wtsessionvar.\wtsid]$ for some $\wtsessionvar$.
%     If $\tsvar = \wttsnone$, then
%     \begin{inparaenum}[\itshape a\upshape)]
%       \item either the transaction $\wtsessionvar.\txn$ has \emph{not} been assigned
%         a commit timestamp
%         (line~\code{\ref{alg:wt-db}}{\ref{line:wtsetcommitts-wttxnglobal-states}})
%       \item or it has been aborted (line~\code{\ref{alg:wt-db}}{\ref{line:wtrollback-wttxnglobal-states}})
%         or locally committed (line~\code{\ref{alg:wt-db}}{\ref{line:wtcommit-wttxnglobal-states}}).
%     \end{inparaenum}
%     Otherwise, $\wtsessionvar.\txn$ has been assigned a commit timestamp
%     but has \emph{not} been locally committed.
%   \item \label{inv:rs-ts-store}
%     Let $\tuple{\txnvar.\tid, \_, \tsvar}$ be a value
%     in $\store[\keyvar]$ for some transaction $\txnvar$ and key $\keyvar$.
%     If $\tsvar \neq \wttsnone$,
%     then $\txnvar$ has been locally committed
%     (line~\code{\ref{alg:wt-db}}{\ref{line:wtcommit-store}}).
% \end{enumerate}
%%%%%%%%%%%%%%%
% \begin{lemma} \label{lemma:rs-majority-commit}
%   Transactions are majority committed
%   in the increasing order of their commit timestamps.
% \end{lemma}
%
% \begin{proof} \label{proof:rs-majority-commit}
%   Due to the replication mechanism (Algorithm~\ref{alg:replication}).
% \end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Visibility Relation} \label{sss:vis-rs}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:visrs}
  \begin{align*}
    &\forall \txnvar_{1}, \txnvar_{2} \in \RSTXN.\;
      \txnvar_{1} \rel{\visrs} \txnvar_{2} \iff \\
      &\qquad \txnvar_{1}.\committs \le \txnvar_{2}.\readts.
  \end{align*}
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-rbaxiom}
  \[
    \ae \models \red{\rbaxiom}.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-rbaxiom}
  Consider two transactions $\txnvar_{1}, \txnvar_{2} \in \RSTXN$
  such that $\txnvar_{1} \rel{\rbrs} \txnvar_{2}$.
  By Lemma~\ref{lemma:rs-majority-commit},
  all transactions with commit timestamps $\le \committs(\txn_{1})$
  have been majority committed and thus locally committed.
  By (\inv \ref{inv:rs-ts-wttxnglobal}),
  all non-$\wttsnone$ $\pinnedcommittedtsvar$ in $\wttxnglobal$
  are larger than $\committs(\txnvar_{1})$
  (line~\code{\ref{alg:wt-db}}{\ref{line:allcommitted-for}})
  when $\txnvar_{2}.\readts$ is computed
  (line\code{\ref{alg:wt-db}}{\ref{line:wtstart-readts}}).
  Therefore, by the way how $\txnvar_{2}.\readts$ is computed
  (line~\code{\ref{alg:wt-db}}{\ref{line:procedure-allcommitted}}),
  $\txnvar_{1}.\committs \le \txnvar_{2}.\readts$.
\end{proof}
%%%%%%%%%%%%%%%

The following lemma shows that the visibility rule for transactions
at the replica set layer amounts to

\hfwei{20210721}{The timestamp overrides WiredTiger ID}

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:visrs-viswt}
  \[
    \visrs \subseteq \red{\viswt???}.
  \]
\end{lemma}
\begin{proof} \label{proof:visrs-viswt}
  Consider two transactions $\txnvar_{1}$ and $\txnvar_{2}$ in $\RSTXN$
  such that $\txnvar_{1} \rel{\visrs} \txnvar_{2}$.
  By Definition~\ref{def:visrs},
  \begin{align}
    \txnvar_{1}.\committs \le \txnvar_{2}.\readts.
    \label{eq:committs-le-readts}
  \end{align}
  We need to show that $\txnvar_{1} \rel{\viswt} \txnvar_{2}$,
  which, by Definition~\ref{def:viswt}, is
  \[
    \committimewt(\txnvar_{1}) < \starttimewt(\txnvar_{2}).
  \]

  Denote by $\timepoint_{1}$ the time
  when $\txnvar_{1}$ obtained its commit timestamp $\txnvar_{1}.\committs$
  (line~\code{\ref{alg:rs-primary}}{\ref{line:rscommit-txn-committs}})
  and atomically set $\txnvar_{1}.\committs$ at the WiredTiger layer
  (line~\code{\ref{alg:wt-db}}{\ref{line:wtsetcommitts-wttxnglobal-states}}).
  Denote by $\timepoint_{2}$ the time $\starttimewt(\txnvar_{1})$
  when $\txnvar_{2}$ computed its read timestamp
  $\txnvar_{2}.\readts$ (line~\code{\ref{alg:wt-db}}{\ref{line:wtstart-readts}}).
  Denote by $\timepoint_{3}$ the time $\committimewt(\txnvar_{1})$
  when $\txnvar_{1}$ was locally committed at the WiredTiger layer
  (line~\code{\ref{alg:wt-db}}{\ref{line:procedure-wtcommit}}).
  See Figure~\ref{fig:thm-visrs-viswt}.
  Note that $\timepoint_{1} < \timepoint_{3}$.

  We first show that
  \[
    \timepoint_{1} < \timepoint_{2}.
  \]
  Suppose by contradiction that $\timepoint_{2} < \timepoint_{1}$.
  By (\inv~\ref{inv:committs-monotonic})
  and the way $\txnvar_{2}.\readts$ is computed,
  we have
  \[
    \txnvar_{2}.\readts < \txnvar_{1}.\committs.
  \]
  A contradiction to (\ref{eq:committs-le-readts}).

  Next we show that
  \[
    \timepoint_{3} < \timepoint_{2},
  \]
  i.e.,
  \[
    \committimewt(\txnvar_{1}) < \starttimewt(\txnvar_{2}).
  \]
  Suppose by contradiction that $\timepoint_{2} < \timepoint_{3}$.
  Since $\timepoint_{1} < \timepoint_{2}$,
  \[
    \timepoint_{1} < \timepoint_{2} < \timepoint_{3}.
  \]
  Thus, at time $\timepoint_{2}$, the condition
  at line~\code{\ref{alg:wt-db}}{\ref{line:allcommitted-pinnedcommittedts}} held.
  By the way $\txnvar_{2}.\readts$ is computed,
  \[
    \txnvar_{2}.\readts < \txnvar_{1}.\committs.
  \]
  A contradiction to (\ref{eq:committs-le-readts}).
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{definition} \label{def:rsvis}
  For a transaction $\txnvar \in \RSTXN$,
  we define $\rsvis(\txnvar)$ to be the set of \rsalg{} transactions
  that are visible to $\txnvar$ according to the visibility rule
  in $\txnvis$ (line~\code{\ref{alg:wt-db}}{\ref{line:procedure-txnvis}}).
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rsvis-welldefined}
  For any transaction $\txnvar \in \RSTXN$,
  $\rsvis(\txnvar)$ is well-defined.
  That is, $\rsvis(\txnvar)$ keeps the same over time.
\end{lemma}
\begin{proof} \label{proof:rsvis-welldefined}
  \hfwei{20210917}{TODO:}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:visrs-rsvis}
  \[
    \visrs^{-1}(\txnvar) = \rsvis(\txnvar).
  \]
\end{lemma}
\begin{proof} \label{proof:visrs-rsvis}
  Consider a transaction $\txnvar \in \RSTXN$.
  By Definition~\ref{def:visrs},
  \[
    \visrs^{-1}(\txnvar) =
      \set{\txnvar' \in \RSTXN \mid \txnvar'.\committs \le \txnvar.\readts}.
  \]
  By line~\code{\ref{alg:wt-db}}{\ref{line:procedure-txnvis}}
  and Lemmas~\ref{lemma:visrs-viswt} and \ref{lemma:rsvis-welldefined},
  \[
    \rsvis^{-1}(\txnvar) =
      \set{\txnvar' \in \RSTXN \mid \txnvar'.\committs \le \txnvar.\readts}.
  \]
  Therefore,
  \[
    \visrs^{-1}(\txnvar) = \rsvis(\txnvar).
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-noconflictaxiom}
  \[
    \ae \models \noconflictaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-noconflictaxiom}
  Consider any two transactions $\txnvar_{1}, \txnvar_{2} \in \RSTXN$
  such that $\txnvar_{1} \conflict \txnvar_{2}$.
  Without loss of generality,
  we suppose that they both update key $\kvar$.
  Suppose by contradiction that
  \[
    \txnvar_{1}.\readts < \txnvar_{2}.\committs
  \]
  and
  \[
    \txnvar_{2}.\readts < \txnvar_{1}.\committs.
  \]
  By Lemma~\ref{lemma:wt-noconflictaxiom},
  $\txnvar_{1}$'s $\wtcommit$ finishes before $\txnvar_{2}$'s $\wtstart$ starts
  or $\txnvar_{2}$'s $\wtcommit$ finishes before $\txnvar_{1}$'s $\wtstart$ starts.
  We thus perform a case analysis.
  \begin{itemize}
    \item \casei: $\txnvar_{1}$'s $\wtcommit$ finishes
      before $\txnvar_{2}$'s $\wtstart$ starts.
      Thus, $\txnvar_{1}$ updates $\kvar$ before $\txnvar_{2}$ does.
      When $\txnvar_{2}$ updates $\kvar$,
      $\tuple{\txnvar_{1}.\tid, \_, \txnvar_{1}.\committs}$ is in $\store[\kvar]$
      (line~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-forall}}).
      The check $\txnvis(\txnvar_{2}, \_, \txnvar_{1}.\committs)$
      (line~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-call-txnvis}}) fails
      because $\txnvar_{1}.\committs > \txnvar_{2}.\readts$
      (line~\code{\ref{alg:wt-db}}{\ref{line:txnvis-invisible}}).
      Therefore, $\txnvar_{2}$ would abort
      (line~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-call-rollback}}).
    \item \caseii: $\txnvar_{2}$'s $\wtcommit$ finishes
      before $\txnvar_{1}$'s $\wtstart$ starts.
      The following argument is similar to \casei.
  \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Arbitrary Relation} \label{sss:rs-ar}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:arrs}
  \begin{align*}
    &\forall \txnvar_{1}, \txnvar_{2} \in \RSTXN.\;
      \txnvar_{1} \rel{\arrs} \txnvar_{2} \iff \\
      &\quad \txnvar_{1}.\committs < \txnvar_{2}.\committs.
  \end{align*}
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:visrs-arrs}
  \[
    \visrs \subseteq \arrs.
  \]
\end{lemma}
\begin{proof} \label{proof:visrs-arrs}
  Consider any two transactions $\txnvar_{1}, \txnvar_{2} \in \RSTXN$
  such that
  \[
    \txnvar_{1} \rel{\visrs} \txnvar_{2}.
  \]
  By Definition~\ref{def:visrs},
  \[
    \txnvar_{1}.\committs \le \txnvar_{2}.\readts.
  \]
  Since
  \[
    \txnvar_{2}.\readts < \txnvar_{2}.\committs,
  \]
  we have
  \[
    \txnvar_{1}.\committs < \txnvar_{2}.\committs.
  \]
  Therefore, by Definition~\ref{def:arrs},
  \[
    \txnvar_{1} \rel{\arrs} \txnvar_{2}.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-prefixaxiom}
  \[
    \ae \models \prefixaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-prefixaxiom}
  Consider transactions $\txnvar_{1}, \txnvar_{2}, \txnvar_{3} \in \RSTXN$
  such that
  \[
    \txnvar_{1} \rel{\arrs} \txnvar_{2} \rel{\visrs} \txnvar_{3}.
  \]
  By Definition~\ref{def:arrs} of $\arrs$
  and Definition~\ref{def:visrs} of $\visrs$,
  \[
    \txnvar_{1}.\committs < \txnvar_{2}.\committs \le \txnvar_{3}.\readts.
  \]
  Therefore, by Definition~\ref{def:visrs} of $\visrs$,
  \[
    \txnvar_{1} \rel{\visrs} \txnvar_{3}.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-conflict-arrs-tid}
  \begin{align*}
    &\forall \txnvar, \txnvar' \in \RSTXN.\; \\
      &\quad \txnvar \conflict \txnvar' \implies (\txnvar \rel{\arrs} \txnvar'
        \iff \txnvar.\tid < \txnvar'.\tid).
  \end{align*}
\end{lemma}
\begin{proof} \label{proof:rs-conflict-arrs-tid}
  Consider any two transactions $\txnvar, \txnvar' \in \RSTXN$
  such that $\txnvar \conflict \txnvar'$.
  By Lemma~\ref{lemma:rs-noconflictaxiom},
  \[
    \txnvar \rel{\visrs} \txnvar' \lor \txnvar' \rel{\visrs} \txnvar.
  \]
  In the following, we proceed in two directions.
  \begin{itemize}
    \item Suppose that $\txnvar \rel{\arrs} \txnvar'$.
      By Lemma~\ref{lemma:visrs-arrs}, it cannot be that
      \[
        \txnvar' \rel{\visrs} \txnvar.
      \]
      Therefore,
      \[
        \txnvar \rel{\visrs} \txnvar'.
      \]
      By Lemma~\ref{lemma:visrs-viswt},
      \[
        \txnvar \rel{\viswt} \txnvar'.
      \]
      By Lemma~\ref{lemma:viswt-tid},
      \[
        \txnvar.\tid < \txnvar'.\tid.
      \]
    \item Suppose that $\txnvar.\tid < \txnvar'.\tid$.
      By Lemma~\ref{lemma:viswt-tid}, it cannot be that
      \[
        \txnvar' \rel{\viswt} \txnvar.
      \]
      By Lemma~\ref{lemma:visrs-viswt}, it cannot be that
      \[
        \txnvar' \rel{\visrs} \txnvar.
      \]
      Therefore,
      \[
        \txnvar \rel{\visrs} \txnvar'.
      \]
      By Lemma~\ref{lemma:visrs-arrs},
      \[
        \txnvar \rel{\arrs} \txnvar'.
      \]
  \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-intaxiom}
  \[
    \ae \models \intaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-intaxiom}
  Consider a transaction $\txnvar \in \RSTXN$.
  Let $\evar = (\_, \readevent(\kvar, \vvar))$
  be an \emph{internal} $\rsread$ operation in $\txnvar$.
  Moreover, $\po^{-1}(\evar) \cap \HEvent_{\evar} \neq \emptyset$.
  Let $\evar' \triangleq \max_{\po}(\po^{-1}(e) \cap \HEvent_{\kvar})$.
  \red{By Lemma~\ref{lemma:rsvis-welldefined}}, compared with $\evar'$,
  no additional update operations on $\kvar$ (from other transactions)
  are visible to $\evar$ at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Thus, $e' = (\_, \_(\kvar, \vvar))$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-extaxiom}
  \[
    \ae \models \extaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-extaxiom}
  Consider a transaction $\txnvar \in \RSTXN$.
  Let $e = (\_, \readevent(k, v))$
  be an \emph{external} $\rsread$ operation in $\txnvar$.
  Consider the set
  $W = \visrs^{-1}(\txnvar) \cap \set{\txnvar \mid \txnvar \vdash \Write k : \_}$
  of transactions that update key $\kvar$ and are visible to $\txnvar$.
  If $W$ is empty, obviously $e$ obtains the initial value of $\kvar$.
  Now suppose that $W \neq \emptyset$.
  By Lemma~\ref{lemma:visrs-rsvis},
  it is also the set of transactions that pass the check of $\txnvis(\txnvar, \_)$
  for key $\kvar$ (line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}).

  % By Lemma~\ref{lemma:rs-noconflictaxiom},
  % the $\visrs$ order among the transactions in $W$ are total.
  % By Lemma~\ref{lemma:visrs-arrs},
  % $\visrs|_{W} = \arrs|_{W}$.
  By Lemma~\ref{lemma:rs-conflict-arrs-tid},
  the $\arrs|_{W}$ order is consistent with the increasing $\tid$ order
  of the transactions in $W$,
  which is the list order at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Therefore, $\max_{\arrs} W \vdash \Write \kvar : \vvar$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem} \label{lemma:rs-cbaxiom}
  \[
    \ae \models \red{\cbaxiom}.
  \]
\end{theorem}
\begin{proof} \label{proof:rs-cbaxiom}
  By Lemma~\ref{lemma:rs-majority-commit},
  \[
    \cbaxiom \subseteq \arrs.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem} \label{thm:rsalg-rtsi}
  \[
    \rsalg \models \rtsi.
  \]
\end{theorem}
\begin{proof} \label{proof:rsalg-rtsi}
  For any history $\h$ of $\rsalg$,
  we construct an abstract execution $\ae = (\h, \visrs, \arrs)$,
  where $\visrs$ and $\arrs$ are given in Definitions~\ref{def:visrs}
  and \ref{def:arrs}, respectively.
  By Lemmas~\ref{lemma:rs-rbaxiom},
  \ref{lemma:rs-noconflictaxiom},
  \ref{lemma:rs-prefixaxiom},
  \red{\ref{lemma:rs-cbaxiom}},
  \ref{lemma:rs-intaxiom}, and
  \ref{lemma:rs-extaxiom},
  $\ae \models \rtsi$.
  Since $\h$ is arbitrary, $\rsalg \models \rtsi$.
\end{proof}
%%%%%%%%%%%%%%%

Additionally, we show that the abstract execution $\ae$
constructed above does not satisfy \inrbaxiom.
%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:rs-not-realtimesnapshot}
  \[
    \ae \not\models \inrbaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:rs-not-realtimesnapshot}
  Example:
  $\txnvar_{1}$ commits \emph{locally}, but has not been majority committed.
  A back-to-back transaction $\txnvar_{2}$ is allowed to observe $\txnvar_{1}$
  (due to speculative majority/snapshot isolation).
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> proofs/sc-correctness.tex <==
% sc-correctness.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness} \label{ss:sc-correctness}

For a relation $R$, we use $R_{\textsc{sc}}$
to denote an instantiation of $R$ specific to the \scalg{} protocol.
Consider a history $\h = (\SCTXN, \sosc)$ of \scalg{},
where we restrict $\SCTXN$ to be set of \emph{committed} transactions.
We prove that $\h$ satisfies \sessionsi{}
by constructing an abstract execution $\ae = (\h, \vissc, \arsc)$.
(Theorem~\ref{thm:scalg-sessionsi})
%%%%%%%%%%%%%%%
\subsubsection{Invariants} \label{sss:sc-invariants}

\begin{enumerate}[(\inv 1)]
  \item \label{inv:sc-}
\end{enumerate}

%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Visibility Relation} \label{sss:vis-sc}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:vissc}
  \begin{align*}
    &\forall \txnvar_{1}, \txnvar_{2} \in \SCTXN.\;
      \txnvar_{1} \rel{\vissc} \txnvar_{2} \iff \\
      &\qquad \txnvar_{1}.\committs \le \txnvar_{2}.\readts.
  \end{align*}
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:sc-session}
  \[
    \ae \models \sessionaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:sc-session}
  Consider two transactions $\txnvar_{1}, \txnvar_{2} \in \SCTXN$
  such that $\txnvar_{1} \rel{\sosc} \txnvar_{2}$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{definition} \label{def:scvis}
  For a transaction $\txnvar \in \SCTXN$,
  we define $\scvis(\txnvar)$ to be the set of \scalg{} transactions
  that are visible to $\txnvar$ according to the visibility rule
  in $\txnvis$ (line~\code{\ref{alg:wt-db}}{\ref{line:procedure-txnvis}}).
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:scvis-welldefined}
  For any transaction $\txnvar \in \SCTXN$,
  $\scvis(\txnvar)$ is well-defined.
  That is, $\scvis(\txnvar)$ keeps the same over time.
\end{lemma}
\begin{proof} \label{proof:scvis-welldefined}
  \hfwei{20211020}{TODO:}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:vissc-scvis}
  \[
    \vissc^{-1}(\txnvar) = \scvis(\txnvar).
  \]
\end{lemma}
\begin{proof} \label{proof:vissc-scvis}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:sc-noconflictaxiom}
  \[
    \ae \models \noconflictaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:sc-noconflictaxiom}
  Consider any two transactions $\txnvar_{1}, \txnvar_{2} \in \SCTXN$
  such that $\txnvar_{1} \conflict \txnvar_{2}$.
  Without loss of generality,
  we suppose that they both update key $\kvar$.
  Suppose by contradiction that
  \[
    \txnvar_{1}.\readts < \txnvar_{2}.\committs
  \]
  and
  \[
    \txnvar_{2}.\readts < \txnvar_{1}.\committs.
  \]
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Arbitrary Relation} \label{sss:sc-ar}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:arsc}
  \begin{align*}
    &\forall \txnvar_{1}, \txnvar_{2} \in \SCTXN.\;
      \txnvar_{1} \rel{\arsc} \txnvar_{2} \iff \\
      &\quad \txnvar_{1}.\committs < \txnvar_{2}.\committs.
  \end{align*}
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:vissc-arsc}
  \[
    \vissc \subseteq \arsc.
  \]
\end{lemma}
\begin{proof} \label{proof:vissc-arsc}
  Consider any two transactions $\txnvar_{1}, \txnvar_{2} \in \SCTXN$
  such that
  \[
    \txnvar_{1} \rel{\visrs} \txnvar_{2}.
  \]
  By Definition~\ref{def:visrs},
  \[
    \txnvar_{1}.\committs \le \txnvar_{2}.\readts.
  \]
  Since
  \[
    \txnvar_{2}.\readts < \txnvar_{2}.\committs,
  \]
  we have
  \[
    \txnvar_{1}.\committs < \txnvar_{2}.\committs.
  \]
  Therefore, by Definition~\ref{def:arsc},
  \[
    \txnvar_{1} \rel{\arsc} \txnvar_{2}.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:sc-prefixaxiom}
  \[
    \ae \models \prefixaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:sc-prefixaxiom}
  Consider transactions $\txnvar_{1}, \txnvar_{2}, \txnvar_{3} \in \SCTXN$
  such that
  \[
    \txnvar_{1} \rel{\arsc} \txnvar_{2} \rel{\vissc} \txnvar_{3}.
  \]
  By Definition~\ref{def:arsc} of $\arsc$
  and Definition~\ref{def:vissc} of $\vissc$,
  \[
    \txnvar_{1}.\committs < \txnvar_{2}.\committs \le \txnvar_{3}.\readts.
  \]
  Therefore, by Definition~\ref{def:visrs} of $\visrs$,
  \[
    \txnvar_{1} \rel{\visrs} \txnvar_{3}.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
% \begin{lemma} \label{lemma:rs-conflict-arrs-tid}
%   \begin{align*}
%     &\forall \txnvar, \txnvar' \in \RSTXN.\; \\
%       &\quad \txnvar \conflict \txnvar' \implies (\txnvar \rel{\arrs} \txnvar'
%         \iff \txnvar.\tid < \txnvar'.\tid).
%   \end{align*}
% \end{lemma}
% \begin{proof} \label{proof:rs-conflict-arrs-tid}
%   Consider any two transactions $\txnvar, \txnvar' \in \RSTXN$
%   such that $\txnvar \conflict \txnvar'$.
%   By Lemma~\ref{lemma:rs-noconflictaxiom},
%   \[
%     \txnvar \rel{\visrs} \txnvar' \lor \txnvar' \rel{\visrs} \txnvar.
%   \]
%   In the following, we proceed in two directions.
%   \begin{itemize}
%     \item Suppose that $\txnvar \rel{\arrs} \txnvar'$.
%       By Lemma~\ref{lemma:visrs-arrs}, it cannot be that
%       \[
%         \txnvar' \rel{\visrs} \txnvar.
%       \]
%       Therefore,
%       \[
%         \txnvar \rel{\visrs} \txnvar'.
%       \]
%       By Lemma~\ref{lemma:visrs-viswt},
%       \[
%         \txnvar \rel{\viswt} \txnvar'.
%       \]
%       By Lemma~\ref{lemma:viswt-tid},
%       \[
%         \txnvar.\tid < \txnvar'.\tid.
%       \]
%     \item Suppose that $\txnvar.\tid < \txnvar'.\tid$.
%       By Lemma~\ref{lemma:viswt-tid}, it cannot be that
%       \[
%         \txnvar' \rel{\viswt} \txnvar.
%       \]
%       By Lemma~\ref{lemma:visrs-viswt}, it cannot be that
%       \[
%         \txnvar' \rel{\visrs} \txnvar.
%       \]
%       Therefore,
%       \[
%         \txnvar \rel{\visrs} \txnvar'.
%       \]
%       By Lemma~\ref{lemma:visrs-arrs},
%       \[
%         \txnvar \rel{\arrs} \txnvar'.
%       \]
%   \end{itemize}
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:sc-intaxiom}
  \[
    \ae \models \intaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:sc-intaxiom}
  Consider a transaction $\txnvar \in \SCTXN$.
  Let $\evar = (\_, \readevent(\kvar, \vvar))$
  be an \emph{internal} $\rsread$ operation in $\txnvar$.
  Moreover, $\po^{-1}(\evar) \cap \HEvent_{\evar} \neq \emptyset$.
  Let $\evar' \triangleq \max_{\po}(\po^{-1}(e) \cap \HEvent_{\kvar})$.
  \red{By Lemma~\ref{lemma:scvis-welldefined}}, compared with $\evar'$,
  no additional update operations on $\kvar$ (from other transactions)
  are visible to $\evar$ at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Thus, $e' = (\_, \_(\kvar, \vvar))$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:sc-extaxiom}
  \[
    \ae \models \extaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:sc-extaxiom}
  Consider a transaction $\txnvar \in \SCTXN$.
  Let $e = (\_, \readevent(k, v))$
  be an \emph{external} $\rsread$ operation in $\txnvar$.
  Consider the set
  $W = \visrs^{-1}(\txnvar) \cap \set{\txnvar \mid \txnvar \vdash \Write k : \_}$
  of transactions that update key $\kvar$ and are visible to $\txnvar$.
  If $W$ is empty, obviously $e$ obtains the initial value of $\kvar$.
  Now suppose that $W \neq \emptyset$.
  By Lemma~\ref{lemma:visrs-rsvis},
  it is also the set of transactions that pass the check of $\txnvis(\txnvar, \_)$
  for key $\kvar$ (line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}).

  % By Lemma~\ref{lemma:rs-noconflictaxiom},
  % the $\visrs$ order among the transactions in $W$ are total.
  % By Lemma~\ref{lemma:visrs-arrs},
  % $\visrs|_{W} = \arrs|_{W}$.
  By Lemma~\ref{lemma:rs-conflict-arrs-tid},
  the $\arrs|_{W}$ order is consistent with the increasing $\tid$ order
  of the transactions in $W$,
  which is the list order at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Therefore, $\max_{\arrs} W \vdash \Write \kvar : \vvar$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem} \label{lemma:rs-cbaxiom}
  \[
    \ae \models \red{\cbaxiom}.
  \]
\end{theorem}
\begin{proof} \label{proof:rs-cbaxiom}
  By Lemma~\ref{lemma:rs-majority-commit},
  \[
    \cbaxiom \subseteq \arrs.
  \]
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem} \label{thm:scalg-sessionsi}
  \[
    \scalg \models \sessionsi.
  \]
\end{theorem}
\begin{proof} \label{proof:scalg-sessionsi}
  For any history $\h$ of $\scalg$,
  we construct an abstract execution $\ae = (\h, \vissc, \arsc)$,
  where $\vissc$ and $\arsc$ are given in Definitions~\ref{def:vissc}
  and \ref{def:arsc}, respectively.
  By Lemmas~\ref{lemma:sc-rbaxiom},
  \ref{lemma:sc-noconflictaxiom},
  \ref{lemma:sc-prefixaxiom},
  \red{\ref{lemma:sc-cbaxiom}},
  \ref{lemma:sc-intaxiom}, and
  \ref{lemma:sc-extaxiom},
  $\ae \models \sessionsi$.
  Since $\h$ is arbitrary, $\scalg \models \sessionsi$.
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> proofs/wt-correctness.tex <==
% wt-correctness.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness} \label{ss:wt-correctness}

For a relation $R$, we use $R_{\textsc{wt}}$
to denote an instantiation of $R$ specific to the \wtalg{} protocol.
Consider a history $\h = (\WTTXN, \sowt)$ of \wtalg{},
where we restrict $\WTTXN$ to be set of \emph{committed} transactions.
We prove that $\h$ satisfies \strongsi{}
by constructing an abstract execution $\ae = (\h, \viswt, \arwt)$
(Theorem~\ref{thm:wtalg-strongsi}).
%%%%%%%%%%%%%%%%%%%%
\subsubsection{Invariants} \label{sss:invariants}

About $\wttxnglobal$
\begin{itemize}
  \item $\forall \wtsidvar \in \WTSID.\; \wttxnglobal[\wtsidvar] \ge 0$
  \item $\wttxnglobal[\wtsessionvar.\wtsid] = \wttidnone$
    means that either $\wtsessionvar$ is \red{idle} or
    the currently active transaction on $\wtsessionvar$
    has not been assigned a transaction identifier yet.
  \item $\wttxnglobal[\wtsessionvar.\wtsid] \neq \wttidnone$
    means that the currently active transaction on $\wtsessionvar$
    has been assigned a transaction identifier.
\end{itemize}

% \begin{enumerate}[(\inv1)]
%   \item \label{inv:committed-txn-tid}
%     For a committed transaction $\txnvar$, $\txnvar.\tid \neq -1$.
% \end{enumerate}
%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Visibility Relation} \label{sss:vis-wt}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:viswt}
  \[
    \viswt \triangleq \rbwt.
  \]
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-rbaxiom}
  \[
    \ae \models \rbaxiom.
  \]
\end{lemma}
% \begin{proof} \label{proof:wt-rbaxiom}
%   By Definition~\ref{def:viswt}, $\rbwt \subseteq \viswt$.
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-realtimesnapshotaxiom}
  \[
    \ae \models \inrbaxiom.
  \]
\end{lemma}
% \begin{proof} \label{proof:wt-realtimesnapshotaxiom}
%   By Definition~\ref{def:viswt}, $\viswt \subseteq \rbwt$.
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:viswt-tid}
  \begin{align*}
    &\forall \txnvar, \txnvar' \in \WTTXN.\; \\
      &\quad \txnvar \rel{\viswt} \txnvar' \implies \txnvar.\tid < \txnvar'.\tid.
  \end{align*}
\end{lemma}
\begin{proof} \label{proof:viswt-tid}
  Consider any two transactions $\txnvar, \txnvar' \in \WTTXN$
  such that $\txnvar \rel{\viswt} \txnvar'$.
  By Definition~\ref{def:viswt},
  \[
    \txnvar \rel{\rbwt} \txnvar'.
  \]
  By lines~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-txn-tid}}
  and \code{\ref{alg:wt-db}}{\ref{line:wtupdate-wttxnglobal-currentid}},
  \[
    \txnvar.\tid < \txnvar'.\tid.
  \]
\end{proof}
%%%%%%%%%%%%%%%

\begin{definition} \label{def:wtvis}
  For a transaction $\txnvar \in \WTTXN$,
  we define $\wtvis(\txnvar)$ to be the set of \wtalg{} transactions
  that are visible to $\txnvar$ according to the visibility rule
  in $\txnvis$ (line~\code{\ref{alg:wt-db}}{\ref{line:procedure-txnvis}}).
\end{definition}

\begin{lemma} \label{lemma:wtvis-welldefined}
  For any transaction $\txnvar \in \WTTXN$,
  $\wtvis(\txnvar)$ is well-defined.
  That is, $\wtvis(\txnvar)$ keeps the same over time.
\end{lemma}
\begin{proof} \label{proof:wtvis-welldefined}
  \hfwei{20210914}{proof}
\end{proof}
%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:viswt-wtvis}
  \[
    \forall \txnvar \in \WTTXN.\; \viswt^{-1}(\txnvar) = \wtvis(\txnvar).
  \]
\end{lemma}
\red{NOTE: $\txnvar.\tid$ changes over time.}
\begin{proof} \label{proof:viswt-wtvis}
  By Definition~\ref{def:viswt} of $\viswt$, we need to show
  \[
    \rbwt^{-1}(\txnvar) = \wtvis(\txnvar).
  \]
  We proceed in two directions.
  \begin{itemize}
    \item $\rbwt^{-1}(\txnvar) \subseteq \wtvis(\txnvar)$.
      Consider a transaction $\txnvar' \in \rbwt^{-1}(\txnvar)$.
      We need to show that $\txnvar'$ is visible to $\txnvar$
      according to the visibility rule.
      \begin{itemize}
        \item Since $\txnvar$ is committed, $\txnvar'.\tid \neq -1$.
        \item By line~\code{\ref{alg:wt-db}}{\ref{line:wtstart-forall-states}},
          $\txnvar'.\tid \notin \txnvar.\concur$.
        \item
      \end{itemize}
    \item $\wtvis(\txnvar) \subseteq \rbwt^{-1}(\txnvar)$.
      Consider a transaction $\txnvar'$ that is visible to $\txnvar$
      according to the visibility rule.
      We need to show that
      \[
        \txnvar' \rel{\rbwt} \txnvar.
      \]
      Suppose by contradiction that
      $\txnvar$ starts \emph{before} $\txnvar'$ commits, i.e.,
      \[
        \starttimewt(\txnvar) < \committimewt(\txnvar').
      \]
      Consider the time $\timepoint'$
      \red{when $\txnvar'$ obtains its identifier}
      \hfwei{20210628}{RO transaction?}
      (line~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-txn-tid}}).
      We distinguish between the following two cases:
      \begin{itemize}
        \item \casei: $\timepoint' < \starttimewt(\txnvar)$.
          By line~\code{\ref{alg:wt-db}}{\ref{line:wtstart-snapshot}},
          \[
            \txnvar'.\tid \in \txnvar.\concur.
          \]
          Thus, by the visibility rule,
          \[
            \txnvar' \notin \wtvis(\txnvar).
          \]
          Contradiction.
        \item \caseii: $\timepoint' > \starttimewt(\txnvar)$.
          By lines~\code{\ref{alg:wt-db}}{\ref{line:wtstart-snapmax}}
          and \code{\ref{alg:wt-db}}{\ref{line:wtupdate-txn-tid}},
          \[
            \txnvar'.\tid \ge \txnvar.\upperlimit.
          \]
          Thus, by the visibility rule,
          \[
            \txnvar' \notin \wtvis(\txnvar).
          \]
        Contradiction.
      \end{itemize}
  \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-noconflictaxiom}
  \[
    \ae \models \noconflictaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:wt-nonconflictaxiom}
  Consider any two transactions $\txnvar, \txnvar' \in \WTTXN$
  such that $\txnvar \conflict \txnvar'$.
  Without loss of generality, we suppose that they both update key $\kvar$,
  and that $\txnvar$ updates $\kvar$ before $\txnvar'$ does.
  Suppose by contradiction that
  neither $\txnvar \rel{\viswt} \txnvar'$
  nor $\txnvar' \rel{\viswt} \txnvar$.
  Consider the time when $\txnvar'$ updates $\kvar$.
  By Lemma~\ref{lemma:viswt-wtvis}, $\txnvar \notin \wtvis(\txnvar')$.
  Thus, $\txnvar'$ would abort
  (line~\code{\ref{alg:wt-db}}{\ref{line:wtupdate-call-txnvis}}).
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Arbitrary Relation} \label{sss:ar-wt}

%%%%%%%%%%%%%%%
\begin{definition} \label{def:arwt}
  \[
    \arwt \triangleq \cbwt.
  \]
\end{definition}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:viswt-arwt}
  \[
    \viswt \subseteq \arwt.
  \]
\end{lemma}
% \begin{proof} \label{proof:viswt-arwt}
%   By Definition~\ref{def:viswt} of $\viswt$
%   and Definition~\ref{def:arwt} of $\arwt$,
%   \[
%     \viswt = \rbwt \subseteq \cbwt = \arwt.
%   \]
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-prefixaxiom}
  \[
    \ae \models \prefixaxiom.
  \]
\end{lemma}
% \begin{proof} \label{proof:wt-prefixaxiom}
%   By Definition~\ref{def:viswt} of $\viswt$,
%   Definition~\ref{def:arwt} of $\arwt$,
%   Definition~\ref{def:rb} of $\rb$,
%   and Definition~\ref{def:cb} of $\cb$,
%   \[
%     \arwt \comp \viswt = \cbwt \comp \rbwt \subseteq \rbwt = \viswt.
%   \]
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-cbaxiom}
  \[
    \ae \models \cbaxiom.
  \]
\end{lemma}
% \begin{proof} \label{proof:wt-cbaxiom}
%   By Definition~\ref{def:arwt}, $\cbwt \subseteq \arwt$.
% \end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-conflict-arwt-tid}
  \begin{align*}
    &\forall \txnvar, \txnvar' \in \WTTXN.\; \\
      &\quad \txnvar \conflict \txnvar' \implies (\txnvar \rel{\arwt} \txnvar'
        \iff \txnvar.\tid < \txnvar'.\tid).
  \end{align*}
\end{lemma}
\begin{proof} \label{proof:wt-conflict-arwt-tid}
  Consider any two transactions $\txnvar, \txnvar' \in \WTTXN$
  such that $\txnvar \conflict \txnvar'$.
  By Lemma~\ref{lemma:wt-noconflictaxiom},
  \[
    \txnvar \rel{\viswt} \txnvar' \lor \txnvar' \rel{\viswt} \txnvar.
  \]
  In the following, we proceed in two directions.
  \begin{itemize}
    \item Suppose that $\txnvar \rel{\arwt} \txnvar'$.
      By Lemma~\ref{lemma:viswt-arwt}, it cannot be that
      \[
        \txnvar' \rel{\viswt} \txnvar.
      \]
      Therefore,
      \[
        \txnvar \rel{\viswt} \txnvar'.
      \]
      By Lemma~\ref{lemma:viswt-tid},
      \[
        \txnvar.\tid < \txnvar'.\tid.
      \]
    \item Suppose that $\txnvar.\tid < \txnvar'.\tid$.
      By Lemma~\ref{lemma:viswt-tid}, it cannot be that
      \[
        \txnvar' \rel{\viswt} \txnvar.
      \]
      Therefore,
      \[
        \txnvar \rel{\viswt} \txnvar'.
      \]
      By Lemma~\ref{lemma:viswt-arwt},
      \[
        \txnvar \rel{\arwt} \txnvar'.
      \]
  \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-intaxiom}
  \[
    \ae \models \intaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:wt-intaxiom}
  Consider a transaction $\txnvar \in \WTTXN$.
  Let $\evar = (\_, \readevent(\kvar, \vvar))$
  be an \emph{internal} $\wtread$ operation in $\txnvar$.
  Moreover, $\po^{-1}(\evar) \cap \HEvent_{\evar} \neq \emptyset$.
  Let $\evar' \triangleq \max_{\po}(\po^{-1}(e) \cap \HEvent_{\kvar})$.
  \red{By Lemma~\ref{lemma:wtvis-welldefined}}, compared with $\evar'$,
  no additional update operations on $\kvar$ (from other transactions)
  are visible to $\evar$ at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Thus, $e' = (\_, \_(\kvar, \vvar))$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:wt-extaxiom}
  \[
    \ae \models \extaxiom.
  \]
\end{lemma}
\begin{proof} \label{proof:wt-extaxiom}
  Consider a transaction $\txnvar \in \WTTXN$.
  Let $e = (\_, \readevent(k, v))$
  be an \emph{external} $\wtread$ operation in $\txnvar$.
  Consider the set
  $W = \viswt^{-1}(\txnvar) \cap \set{\txnvar \mid \txnvar \vdash \Write k : \_}$
  of transactions that update key $\kvar$ and are visible to $\txnvar$.
  If $W$ is empty, obviously $e$ obtains the initial value of $\kvar$.
  Now suppose that $W \neq \emptyset$.
  By Lemma~\ref{lemma:viswt-wtvis},
  it is also the set of transactions that pass the check of $\txnvis(\txnvar, \_)$
  for key $\kvar$ (line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}).

  % By Lemma~\ref{lemma:wt-noconflictaxiom},
  % the $\viswt$ order among the transactions in $W$ are total.
  % By Lemma~\ref{lemma:viswt-arwt},
  % $\viswt|_{W} = \arwt|_{W}$.
  By Lemma~\ref{lemma:wt-conflict-arwt-tid},
  the $\arwt|_{W}$ order is consistent with the increasing $\tid$ order
  of the transactions in $W$,
  which is the list order at line~\code{\ref{alg:wt-db}}{\ref{line:wtread-call-txnvis}}.
  Therefore, $\max_{\arwt} W \vdash \Write \kvar : \vvar$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem} \label{thm:wtalg-strongsi}
  \[
    \wtalg \models \strongsi.
  \]
\end{theorem}
\begin{proof} \label{proof:wtalg-strongsi}
  For any history $\h$ of $\wtalg$,
  we construct an abstract execution $\ae = (\h, \viswt, \arwt)$,
  where $\viswt$ and $\arwt$ are given in Definitions~\ref{def:viswt}
  and \ref{def:arwt}, respectively.
  By Lemmas~\ref{lemma:wt-rbaxiom}, \ref{lemma:wt-realtimesnapshotaxiom},
  \ref{lemma:wt-noconflictaxiom},
  \ref{lemma:wt-prefixaxiom},
  \ref{lemma:wt-cbaxiom},
  \ref{lemma:wt-intaxiom}, and
  \ref{lemma:wt-extaxiom},
  $\ae \models \strongsi$.
  Since $\h$ is arbitrary, $\wtalg \models \strongsi$.
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/ack.tex <==
% ack.tex

\section{Acknowledgments}


==> sections/app-impl.tex <==
% app-impl.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementations} \label{section:app-impl}

\input{tables/table-src}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/discussion.tex <==
% discussion.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion} \label{section:discussion}

%%%%%%%%%%%%%%%%%%%%
\subsection{Concurrency} \label{ss:concurrency}

We will consider intra-process concurrency and the locking mechanisms in the future work. Now we illustrate how our assumption simplifies the pseudocode.

% Consider the calculation of $\snapshot$ of transaction $\txnvar$
% on session $\wtsessionvar$ during \wtstart{}
% (lines~\code{\ref{alg:wt-db}}{\ref{line:wtstart-forall-states}}--\code{\ref{alg:wt-db}} {\ref{line:wtstart-snapshot}}). \red{As argued in Section~\ref{ss:wt-correctness}}, [ \wtsidvar \neq \wtsessionvar.\wtsid \land 0 < \tidvar < \currenttidvar ] vs. [ \tidvar \neq 0 ]
%%%%%%%%%%%%%%%%%%%%
\subsection{Failure} \label{ss:failure}

\begin{itemize}
  \item 2PC variant always commits
\end{itemize}
%%%%%%%%%%%%%%%%%%%%
\subsection{Conformance to Implementations} \label{ss:conformance}

Model-based testing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tables/table-notations.tex <==
% notations.tex

\begin{table}[t]
  \centering
  \caption{Notations}
  \label{table:notations}
  \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{|c|c|c|}
    \hline
    Category   & Notation & Meaning  \\ \hline \hline
    \multirow{6}{*}{Consistency Models}
      & $\T$ & the set of all transactions \\ \cline{2-3}
      & $\txnvar$& transaction                  \\ \cline{2-3}
      & $\Key$   & the set of all possible keys \\ \cline{2-3}
      & $\keyvar$& key                          \\ \cline{2-3}
      & $\Val$   & the set of all possible values \\ \cline{2-3}
      & $\valvar$& value                        \\ \cline{2-3}
      &          &                              \\ \hline \hline
    \multirow{2}{*}{\wtalg}
      & $\WTTXN$
      & \incell{c}{the set of all transactions \\ at the WiredTiger layer}
      \\ \cline{2-3}
      &          &
      \\ \hline \hline
    \multirow{2}{*}{\rsalg}
      & $\RSTXN$
      & \incell{c}{the set of all transactions \\ at the ReplicaSet layer}
      \\ \cline{2-3}
      &          &
      \\ \hline \hline
    \multirow{2}{*}{\scalg}
      & $\SCTXN$
      & \incell{c}{the set of all transactions \\ at the ShardedCluster layer}
      \\ \cline{2-3}
      & &
      \\ \hline
    \end{tabular}}
\end{table}


==> tables/table-src.tex <==
% table-src.tex

\begin{table}[t]
  \centering
  \caption{Pseudocode and Source Code}
  \label{table:pseudocode-src}
  \resizebox{0.50\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|}
    	\hline
    	\multicolumn{2}{|c|}{Pseudocode}                                 & \multicolumn{2}{c|}{Source Code} &  &  \\ \hline
    	       Algorithm        & $\textsf{variable}$/\textsc{Procedure} & File &       Field/Method        &  &  \\ \hline
    	\multirow{5}{*}{\wtalg} &                $\store$                &      &                           &  &  \\ \cline{2-6}
    	                        &               $\wtstart$               &      &                           &  &  \\ \cline{2-6}
    	                        &               $\wtread$                &      &                           &  &  \\ \cline{2-6}
    	                        &              $\wtupdate$               &      &                           &  &  \\ \cline{2-6}
    	                        &              $\wtcommit$               &      &                           &  &  \\ \cline{2-6}
    	                        &             $\wtrollback$              &      &                           &  &  \\ \cline{2-6}
    	                        &               $\txnvis$                &      &                           &  &  \\ \cline{2-6}
    	                        &            $\allcommitted$             &      &                           &  &  \\ \cline{2-6}
    	                        &             $\wtsetreadts$             &      &                           &  &  \\ \cline{2-6}
    	                        &            $\wtsetcommitts$            &      &                           &  &  \\ \cline{2-6}
    	                        &              $\wtprepare$              &      &                           &  &  \\ \cline{2-6}
    	                        &          $\wtcommitpreparets$          &      &                           &  &  \\ \cline{2-6}
    	                        &           $\wtcommitprepare$           &      &                           &  &  \\ \hline
    	\multirow{4}{*}{\rsalg} &                                        &      &                           &  &  \\ \cline{2-6}
    	                        &                                        &      &                           &  &  \\ \cline{2-6}
    	                        &                                        &      &                           &  &  \\ \hline
    	\multirow{4}{*}{\scalg} &                                        &      &                           &  &  \\ \cline{2-6}
    	                        &                                        &      &                           &  &  \\ \cline{2-6}
    	                        &                                        &      &                           &  &  \\ \hline
    \end{tabular}}
\end{table}

